Modal Effect Types

Effect handlers are a powerful abstraction for defining, customising, and composing computational effects. Statically ensuring that all effect operations are handled requires some form of effect system, but using a traditional effect system would require adding extensive effect annotations to the millions of lines of existing code in these languages. Recent proposals seek to address this problem by removing the need for explicit effect polymorphism. However, they typically rely on fragile syntactic mechanisms or on introducing a separate notion of second-class function. We introduce a novel approach based on modal effect types.

==> Makefile <==
LATEXMK := $(shell command -v latexmk 2> /dev/null)

TEXC=pdflatex
CFLAGS=-interaction=nonstopmode -halt-on-error -file-line-error
BIBC=bibtex
PAPER=ergonomic-effects
BIBLIO=reference

# Sam wants to use latexmk -- I don't. You can opt out of using
# latexmk by adding your username to the array OPT_OUT below.
BUILD_METHOD=$(PAPER).pdf
OPT_OUT := dhil

all:
  ifndef LATEXMK
    BUILD_METHOD=$(PAPER).pdf
  else
    ifneq ($(filter $(USER),$(OPT_OUT)),)
      BUILD_METHOD=$(PAPER).pdf
    else
      BUILD_METHOD=$(PAPER).pdf-via-latexmk
    endif
  endif
all: $(BUILD_METHOD)

extended: $(BUILD_METHOD)-extended
arxiv: $(BUILD_METHOD)-arxiv
camera-ready: all


crop: $(PAPER).pdf
	pdftk $(PAPER).pdf cat 1-29 output submission.pdf

$(PAPER).aux: $(PAPER).tex
	$(TEXC) $(CFLAGS) $(PAPER)

$(BIBLIO).bbl: $(PAPER).aux $(BIBLIO).bib
	$(BIBC) $(PAPER)

$(PAPER).pdf-arxiv: CFLAGS:=$(CFLAGS) "\def\ARXIV{}\input{$(PAPER)}"
$(PAPER).pdf-arxiv: all

$(PAPER).pdf-extended: CFLAGS:=$(CFLAGS) "\def\EXTENDED{}\input{$(PAPER)}"
$(PAPER).pdf-extended: all

$(PAPER).pdf: $(PAPER).aux $(BIBLIO).bbl
	$(TEXC) $(CFLAGS) $(PAPER)
	$(TEXC) $(CFLAGS) $(PAPER)

$(PAPER).pdf-via-latexmk: $(PAPER).tex
	latexmk -pdf $(CFLAGS) $(PAPER)

$(PAPER).pdf-via-latexmk-extended: $(PAPER).tex
	latexmk -pdf -pdflatex='pdflatex %O $(CFLAGS) -synctex=1 "\def\EXTENDED{}\input{%S}"' $(PAPER)

$(PAPER).pdf-via-latexmk-arxiv: $(PAPER).tex
	latexmk -pdf -pdflatex='pdflatex %O $(CFLAGS) -synctex=1 "\def\ARXIV{}\input{%S}"' $(PAPER)

clean:
	rm -f *.log *.aux *.toc *.out
	rm -f *.bbl *.blg *.fls *.xml
	rm -f *.fdb_latexmk *.vtc *.cut
	rm -f $(PAPER).pdf camera-ready.pdf submission.pdf
	rm -f *.o *.cmx *.cmo

